Filter Learning for Subgraphs: Algebras and Performance Risk Bounds

Graph signal processing tasks that leverage spectral information typically assume access to the complete graph topology, which is often unavailable in practice. We propose a systematic framework for subgraph filter learning (SFL), where subgraph-supported operators approximate ambient graph filters under partial observations. We formulate SFL as a statistical learning problem in which optimal subgraph operators are inherently data-dependent. To address the difficulty of directly estimating such operators, we develop a subgraph filter algebra based on distance-aware Laplacian constructions, defining a structured and controllable class of filters for effective approximation. We further establish performance risk bounds under the least squares loss, quantifying how well the learned operator approximates the restricted ambient mapping. Experiments real-world datasets show that, for SFL tasks, the proposed algebraic models consistently outperform polynomial filters, distribution-agnostic operators, and direct numerical filter learning baselines that attempt to recover the underlying structure from data.

==> latexmkrc <==
ensure_path( 'BIBINPUTS', './bib//' );
ensure_path( 'TEXINPUTS', './latex//' ); # E.g., path to directory containing your preamble.tex

##########################################
# #For use in Overleaf with xr package
##########################################

$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ('-cd', '-interaction=nonstopmode', '-file-line-error');

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    my $target = $_[0];
    # Track files currently being built (prevents circular dependencies)
    # and files already built (compile each file only once per session)
    our %building_stack;
    our %already_built;
    
    # Skip if: same as root, currently being built, or already compiled
    if (defined($root_filename) && 
        ($root_filename ne $target) && 
        !$building_stack{$target} && 
        !$already_built{$target}) {
        
        $building_stack{$target} = 1;
        system("latexmk -cd -pdf \"$target\"");
        delete $building_stack{$target};
        $already_built{$target} = 1;
    }
}

##########################################
##########################################
